Going In Blind: Object Motion Classification using Distributed Tactile Sensing for Safe Reaching in Clutter

Robotic manipulators navigating cluttered shelves or cabinets may find it challenging to avoid contact with obstacles. Indeed, rearranging obstacles may be necessary to access a target. Rather than planning explicit motions that place obstacles into a desired pose, we suggest allowing incidental contacts to rearrange obstacles while monitoring contacts for safety. Bypassing object identification, we present a method for categorizing object motions from tactile data collected from incidental contacts with a capacitive tactile skin on an Allegro Hand. We formalize tactile cues associated with categories of object motion, demonstrating that they can determine with $>90$% accuracy whether an object is movable and whether a contact is causing the object to slide stably (safe contact) or tip (unsafe).

==> IROS 2022 -- Object Mobi/sections/sensorDesignRearrangement.tex <==
We now consider the design requirements for sensory skins intended to provide information about incidental contacts, focusing on classifying object motions, and present a new distributed tactile sensor network for the Allegro Hand. The skin used in this work is a modified version of the fringe field mutual capacitance sensor presented in \cite{ruth2021flexible}. The elements comprising each sensor in the network are outlined in Fig.~\ref{fig:sensor-design}A. A flexible PCB contains 3x3\,mm taxels with an interdigitated design arranged in a matrix. The electrodes are connected to the capacitance-to-digital converter of a Cypress PsoC 4200 microcontroller, which translates capacitance to signal counts. Pressure is transformed to a change in mutual capacitance through the addition of a textured dielectric which, when compressed, increases the effective dielectric constant as air is displaced. The textured dielectric is molded from urethane (SmoothOn Vytaflex-30) and features cylindrical pillars (0.8\,mm diameter, 0.8\,mm height). The dielectric is fixed to the electrode using a 1.6\,mm thick adhesive-backed silicone encapsulation layer. 

Contact localization is essential for determining how the robot should move in response to a contact. Especially when covering large areas, there is a trade-off between spatial resolution and sampling rate. In this work, we present experiments conducted with a back of hand sensor, 
% which is able to resolve contacts to within \todo{FILL IN cm}
which contains four taxels per $\text{cm}^2$ and has a sampling rate of 10\,Hz. Figure~\ref{fig:sensor-design}C shows the sensor's response to loading and unloading up to 50\,N as force is applied with a 12\,mm diameter probe. For a point contact (1.9\,mm diameter probe), the sensor can detect forces as light as 0.06\,N. 


\subsection{Design Considerations for Interaction in Cluttered Spaces}
\subsubsection{Coverage}
Although contacts during grasping and manipulation may be constrained to specific areas of the hand, contacts during reaching often occur on the backside of the hand, especially if reaching with fingers slightly flexed. To avoid undetected contacts, the skin should ideally cover the entire hand. The coverage achieved by our sensor network is displayed in Fig. \ref{fig:sensor-design}B. 

\subsubsection{Curvature}
While flat tactile sensors are easier to manufacture, curvature is beneficial for capturing and tracking incidental contact events. As shown in Fig.~\ref{fig:curved-sensor}, flat sensors provide large contact areas when aligned with a surface, but are prone to quickly losing contact when there is any misalignment, such as the onset of tip. Adding curvature to the sensor in the direction of gravity leads to contacts which travel down the surface of the sensor as an object tips. 

We develop a 2D kinematic model for contact point motion as a curved sensor tips an object. This will later be used to determine appropriate tactile cues for tip events. For a sensor with radius of curvature $R$ contacting a vertically uniform object of width $w$, one can determine the tip angle, $\theta$, of the object by solving the vector loop equation set up in Fig.~\ref{fig:curved-sensor}. We define two right-handed orthonormal bases: $\hat{n}_{xyz}$ and $\hat{b}_{xyz}$, fixed to the world and object, respectively. Unit vector $\hat{n}_x$ points along the ground and $\hat{n}_y$ points vertically upward and, initially, $\hat{b}_x = \hat{n}_x$ and $\hat{b}_y = \hat{n}_y$. The sensor contacts the object at height $h$ and moves along $\hat{n}_x$ a distance of $x$, causing the object to tip by $\theta$. We write a vector loop beginning and ending at $P$, the center of curvature of the sensor when it initially contacts the object, to obtain
%No new paragraph!  -MRC
\begin{equation}
    x \hat{n}_x + R \hat{b}_x - y \hat{b}_y + w \hat{b}_x - (R + w)\hat{n}_x = \Vec{0}. 
    \label{eqn:loop}
\end{equation}
Taking the dot product of eq.~\ref{eqn:loop} with $\hat{n}_x$ and $\hat{n}_y$ produces two scalar equations which can be solved for $\theta$. The distance we expect the contact to move in the gravity direction can then be calculated as $R \theta$. Smaller radii may require a larger tip angle before contact patch motion indicating tip is detectable but larger radii will lose contact with a tipping object faster. The sensor used in experiments features a gentle curvature with a radius of 372\,mm. 

\begin{figure}[thb]
\vspace{5pt}
  \centering
  \includegraphics[width=\linewidth]{figures/curved_sensor_tip_horizontal.png}
  \caption{Curved surfaces are beneficial for sensing tipping. A schematic illustrates the vector loop in eq.~\ref{eqn:loop}.}
  \label{fig:curved-sensor}
  \vspace{-12pt}
\end{figure}


